PFGM++: Unlocking the Potential of Physics-Inspired Generative Models

We introduce a new family of physics-inspired generative models termed PFGM++ that unifies diffusion models and Poisson Flow Generative Models (PFGM). These models realize generative trajectories for $N$ dimensional data by embedding paths in $N{+}D$ dimensional space while still controlling the progression with a simple scalar norm of the $D$ additional variables. The new models reduce to PFGM when $D{=}1$ and to diffusion models when $D{\to}\infty$. The flexibility of choosing $D$ allows us to trade off robustness against rigidity as increasing $D$ results in more concentrated coupling between the data and the additional variable norms. We dispense with the biased large batch field targets used in PFGM and instead provide an unbiased perturbation-based objective similar to diffusion models. To explore different choices of $D$, we provide a direct alignment method for transferring well-tuned hyperparameters from diffusion models ($D{\to} \infty$) to any finite $D$ values. Our experiments show that models with finite $D$ can be superior to previous state-of-the-art diffusion models on CIFAR-10/FFHQ $64{\times}64$ datasets, with FID scores of $1.91/2.43$ when $D{=}2048/128$. In class-conditional setting, $D{=}2048$ yields current state-of-the-art FID of $1.74$ on CIFAR-10. In addition, we demonstrate that models with smaller $D$ exhibit improved robustness against modeling errors. Code is available at https://github.com/Newbeeer/pfgmpp

==> perturbation_kernel.tex <==
\label{sec:perturbed-kernel}

The objective inherited from PFGM paper~\cite{Xu2022PoissonFG} requires sampleing a large batch of data from $\{\rvy_i\}_{i=1}^n \sim {p}^n({\rvy})$ in each updates to approximate the integral in the electric field~(\Eqref{eq:poisson-field-D}):
\begin{align*}
&\E_{\tilde{p}_{\textrm{train}}(\tx)}\E_{\{\rvy_i\}_{i=1}^n\sim p^n(\rvy)}\E_{\rvx\sim p_\sigma(\rvx|\rvy_1)}\\
&\qquad\left[\Big\lVert f_{\theta}(\tilde{\rvx})- \frac{\sum_{i=0}^{n-1} \frac{\tilde{\mat{x}}-\Tilde{\rvy}_i}{||\tilde{\mat{x}}-\Tilde{\rvy}_i||^{N+D}}}{||\sum_{i=0}^{n-1} \frac{\tilde{\mat{x}}-\Tilde{\rvy}_i}{||\tilde{\mat{x}}-\Tilde{\rvy}_i||^{N+D}}||_2+\gamma}\Big\rVert^2_2 \right]
\end{align*}
where $\tilde{p}_{\textrm{train}}$ is heuristically designed to cover the regions that the backward ODE traverses. The objective has several obvious drawbacks: \textit{(1)} The large batch incurs additional overheads; \textit{(2)} Its minimizer is biased estimator of the electric field~(\Eqref{eq:poisson-field-D}); \textit{(3)} The large batch is incompatible with typical conditional generation setups, where each condition only contains one samples, such as text-to-image~\cite{Rombach2021HighResolutionIS, Ramesh2022HierarchicalTI,Saharia2022PhotorealisticTD} and text-to-3D generation~\cite{Poole2022DreamFusionTU}.

In this section, we present a new objective for learning the electric field without the need for a large batch, through special design of perturbation kernel. The objective has unbiased minimizer and enables one-sample-per-condition generation.

\subsection{Design of perturbation kernel}
Inspired by denoising score-matching~\cite{Vincent2011ACB}, we can carefully design the perturbation kernel to ensure the minimizer in the following square loss matches the ground-truth electric field in \Eqref{eq:poisson-field-D}:
\begin{align*}
    \E_{r\sim p(r)}\E_{p({\rvy})}\E_{p_{r}(\rvx|{\rvy})}\left[|| f_{\theta}(\tilde{\rvx})- ({{\tilde{\rvx}-\tilde{\rvy}}})||_2^2\right] \numberthis \label{eq:new-D-aug}
\end{align*}
where $p(r)$ is training distributions of $r$ supported on $(0, \infty)$, and $p_{r}(\rvx|{\rvy})$ is the perturbation kernel to be determined. Recall that the clean data $\ty = (\rvy,0)$ and the perturbed data $\tx=(\rvx, r)$. One can show that the  minimizer of \Eqref{eq:new-D-aug} is $f^*_{\theta}(\tilde{\rvx}) \propto {\int p_r(\rvx|{{\rvy}})({\tilde{\rvx}-\tilde{\rvy}})p({\rvy}) \mathrm{d}{\rvy}}$, which in turn can match the direction of electric field $\mat{E}(\tilde{\mat{x}}) \propto \int {\tilde{\mat{x}}-\tilde{\rvy}}/{||\tilde{\mat{x}}-\tilde{\rvy}||^{N+D}}{p}({\rvy}) \mathrm{d} {\rvy}$ when setting $p_{r}(\rvx|{\rvy}) \propto {1}/{||\tx - \tilde{\rvy}||^{N+D}} =  {1}/{({||\rvx-{\rvy}||_2^2+ r^2})^\frac{N+D}{2}}$. Consequently, the $r$-dependent marginal distribution as $p_r(\rvx) = \int p_r(\rvx|\rvy)p(\rvy)d\rvy$. The following proposition states that the choice ensures the minimizer in the square loss matches the direction of electric field.
\begin{restatable}{proposition}{thmmin}
\label{thm:minimizer}
    With perturbation kernel $p_{r}(\rvx|{\rvy}) \propto {1}/{({||\rvx-{\rvy}||_2^2+ r^2})^\frac{N+D}{2}}$, for $\forall \rvx\in \R^N, r>0$, the minimizer $f^*_\theta(\tx)$ in the PFGM++ objective~(\Eqref{eq:new-D-aug}) matches the direction of electric field $\mat{E}(\tx)$ in \Eqref{eq:poisson-field-D}. Specifically, 
$
        f^*_\theta(\tx) = ({S_N(1)}/{p_r(\rvx)})\mat{E}(\tx)
$.
\end{restatable}
% \begin{proofs}
% The minimizer at $\tx$ in \Eqref{eq:new-D-aug} is
% \begin{align*}
%     f^*_{\theta}(\tilde{\rvx}) &= \frac{\int p_r(\rvx|{{\rvy}})({\tilde{\rvx}-\tilde{\rvy}})p({\rvy}) d{\rvy}}{p_r(\rvx)}
% \end{align*}
% By substituting the expression of perturbation kernel $p_{r}(\rvx|{\rvy})$, we immediately arrive at the results.
% \end{proofs}
We defer the proof to Appendix~\ref{app:thm-minimizer}. The theorem indicates that the minimizer $f^*_\theta(\tx)$ can match the direction of $\mat{E}(\tx)$ with sufficient data and model capacity. The current training target for the neural network is the directional vector between the clean data $\ty$ and perturbed data $\tx$ akin to denoising score-matching for diffusion models~\cite{Song2021ScoreBasedGM, Karras2022ElucidatingTD}. In addition, the new objective allows for conditional generation under one-sample-per-condition setup. Since the perturbation kernel is isotropic, we can decompose $p_r(\cdot|\rvy)$ in hyperspherical coordinates to $\gU_{\psi}(\psi)p_r(R)$, where $\gU_{\psi}$ is the uniform distribution over the angle component. The distribution of the perturbed radius $R=||\rvx - \rvy||_2$ is
\begin{align*}
    p_r(R) \propto \frac{R^{N-1}}{({R^2+ r^2})^\frac{N+D}{2}}
\end{align*}
We defer the practical sampling procedure of the perturbation kernel to Appendix~\ref{app:sample-prior}. The mean of the $r$-dependent radius distribution $p_r(R)$ is about $r\sqrt{N/(D-2)}$. Hence we explicitly normalize the target in \Eqref{eq:new-D-aug} by $r/\sqrt{D}$, to keep the norm of the target output near the constant $\sqrt{N}$, similar to diffusion models~\cite{Song2021ScoreBasedGM}. In addition, we drop the last dimension of the target because it is a constant ---  $({\tilde{\rvx}-\tilde{\rvy}})_{r}/({r}/{\sqrt{D}})=\sqrt{D}$. Together, the new objective is
\begin{align*}
    \E_{r\sim p(r)}\E_{p(\tilde{\rvy})}\E_{p_{r}(\tx|\tilde{\rvy})}\left[\Big\lVert f_{\theta}(\tilde{\rvx})- \frac{{\rvx}-{\rvy}}{{r}/{\sqrt{D}}}\Big\rVert_2^2\right] \numberthis \label{eq:pfgmpp-obj}
\end{align*}
After training the neural network through objective \Eqref{eq:pfgmpp-obj}, we can use the ODE~(\Eqref{eq:ode-pfgmpp}) anchored by $r$ to generate samples, \ie $\mathrm{d}\rvx /\mathrm{d}r = f_\theta(\tx) / \sqrt{D}$ with prior distribution $p_{\rmax}$.


